Development of an indoor localization and navigation system based on monocular SLAM for mobile robots

Localization and navigation are two crucial issues for mobile robots. In this paper, we propose an approach for localization and navigation systems for a differential-drive robot based on monocular SLAM. The system is implemented on the Robot Operating System (ROS). The hardware includes a differential-drive robot with an embedded computing platform (Jetson Xavier AGX), a 2D camera, and a LiDAR sensor for collecting external environmental information. The A* algorithm and Dynamic Window Approach (DWA) are used for path planning based on a 2D grid map. The ORB_SLAM3 algorithm is utilized to extract environmental features, providing the robot's pose for the localization and navigation processes. Finally, the system is tested in the Gazebo simulation environment and visualized through Rviz, demonstrating the efficiency and potential of the system for indoor localization and navigation of mobile robots.

==> vncaps.tex <==
% Copyright 2000-2006 Werner Lemberg <wl@gnu.org> and
%                     Han The Thanh <hanthethanh@gmx.net>.
% This file is part of vntex.  License: LPPL, version 1.3 or newer,
% according to http://www.latex-project.org/lppl.txt

\ifx\ProvidesFile\undefined \else
  \ProvidesFile{vncaps.tex}[2006/06/07 v1.1 Captions in Vietnamese]  
\fi
 
% Vietnamese captions; edit them in viscii/tcvn/utf8, then use
% `vntovn viscii vntex' or a similar command to convert to vntex.
%
% History
%
% ????/??/??:
%     Split off captions from vietnam.ldf.
%     Add \captionsenglish, \dateUSenglish, and \dateenglish.
%
% 2005/04/21:
%     Add copyright message.
%     Don't use `{}' but a space after macros which don't have arguments.
%
% 2006/06/07:
%     Fix bug in \indexname.  Add version number.

\ifx\providecommand \undefined
  \let\providecommand \def
\fi

\providecommand\captionsvietnam{% 
  \def\prefacename{L\`\ohorn i n\'oi \dj\`\acircumflex u}%
%  \def\refname{T\`ai li\d\ecircumflex u}%
  \def\Acknowledgmentname{L\`\ohorn i c\h{a}m \ohorn n}%
  \def\refname{T\`ai li\d\ecircumflex u tham kh\h{a}o}%
%  \def\abstractname{T\'om t\'\abreve t n\d\ocircumflex i dung}
  \def\abstractname{T\'om t\'\abreve t}
  \def\IEEEkeywordsname{T\`\uhorn \, kh\'oa}
  \def\bibname{T\`ai li\d\ecircumflex u tham kh\h{a}o}%
  \def\chaptername{Ch\uhorn \ohorn ng}%
  \def\appendixname{Ph\d{u} l\d{u}c}%
  \def\contentsname{M\d{u}c l\d{u}c}%
  \def\listfigurename{Danh s\'ach h\`inh v\~e}%
  \def\listtablename{Danh s\'ach b\h{a}ng}%
  \def\indexname{Ch\h{i} m\d{u}c}% 
  \def\figurename{H\`inh}%
  \def\tablename{B\h{a}ng}%
  \def\partname{Ph\`\acircumflex n}%
  \def\pagename{Trang}%
  \def\headpagename{Trang}%
  \def\seename{Xem}%
  \def\alsoname{Xem th\ecircumflex m}%
  \def\enclname{K\`em theo}%
  \def\ccname{C\`ung g\h\uhorn i}%
  \def\headtoname{G\h\uhorn i}%
  \def\proofname{Ch\'\uhorn ng minh}}

\providecommand\datevietnam{%
  \def\today{%
    Ng\`ay \number\day\space
    th\'ang \number\month\space
    n\abreve m \number\year}}

\providecommand\captionsenglish{%
  \def\prefacename{Preface}%
  \def\refname{References}%
  \def\abstractname{Abstract}%
  \def\bibname{Bibliography}%
  \def\chaptername{Chapter}%
  \def\appendixname{Appendix}%
  \def\contentsname{Contents}%
  \def\listfigurename{List of Figures}%
  \def\listtablename{List of Tables}%
  \def\indexname{Index}%
  \def\figurename{Figure}%
  \def\tablename{Table}%
  \def\partname{Part}%
  \def\enclname{encl}%
  \def\ccname{cc}%
  \def\headtoname{To}%
  \def\pagename{Page}%
  \def\headpagename{Page}%
  \def\prefacename{Preface}%
  \def\seename{see}%
  \def\alsoname{see also}}

\providecommand\dateenglish{%
  \def\today{%
    \ifcase\day\or 1st\or 2nd\or 3rd\or 4th\or 5th\or 6th\or 7th\or
    8th\or 9th\or 10th\or 11th\or 12th\or 13th\or 14th\or 15th\or
    16th\or 17th\or 18th\or 19th\or 20th\or 21st\or 22nd\or 23rd\or
    24th\or 25th\or 26th\or 27th\or 28th\or 29th\or 30th\or 31st\fi
    ~\ifcase\month\or January\or February\or March\or April\or May\or
    June\or July\or August\or September\or October\or November\or
    December\fi \space
    \number\year}}

\providecommand\dateUSenglish{%
  \def\today{%
    \ifcase\month\or January\or February\or March\or April\or May\or
    June\or July\or August\or September\or October\or November\or
    December\fi \space\number\day, \number\year}}

\endinput

% end of vncaps.tex

